Emergence of highly coherent quantum subsystems of a noisy and dense spin system

Quantum sensors and qubits are usually two-level systems (TLS), the quantum analogs of classical bits which assume binary values '0' or '1'. They are useful to the extent to which they can persist in quantum superpositions of '0' and '1' in real environments. However, such TLS are never alone in real materials and devices, and couplings to other degrees of freedom limit the lifetimes - called decoherence times - of the superposition states. Decoherence occurs via two major routes - excitation hopping and fluctuating electromagnetic fields. Common mitigation strategies are based on material improvements, exploitation of clock states which couple only to second rather than first order to external perturbations, and reduction of interactions via extreme dilution of pure materials made from isotopes selected to minimize noise from nuclear spins. We demonstrate that for a dense TLS network in a noisy nuclear spin bath, we can take advantage of interactions to pass from hopping to fluctuation dominance, increasing decoherence times by almost three orders of magnitude. In the dilute rare-earth insulator LiY1-xTbxF4, Tb ions realize TLS characterized by a 30GHz splitting and readily implemented clock states. Dipolar interactions lead to coherent, localized pairs of Tb ions, that decohere due to fluctuating quantum mechanical ring-exchange interaction, sensing the slow dynamics of the surrounding, nearly localized Tb spins. The hopping and fluctuation regimes are sharply distinguished by their Rabi oscillations and the invisible vs. strong effect of classic 'error correcting' microwave pulse sequences. Laying open the decoherence mechanisms at play in a dense, disordered and noisy network of interacting TLS, our work expands the search space for quantum sensors and qubits to include clusters in dense, disordered materials, that can be explored for localization effects.

==> SuppMat/Parameters.tex <==
% Optical absorption measurements by the manufacturer at 487\,nm yielded $0.1\%$ and $0.004\%$ respectively. Rutherford backscattering confirmed the $x=0.09\pm0.002\%$ for the denser sample.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pulse configurations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
% B=38mT wide range frEq.scan 50MHz res.
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.244	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	500.	200.	0.244	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	1200.	1024.	1.5								
% digrate	2.										

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 26.	380.	1.*10^6	20.	1.	80.	1.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% B=38mT narrow range freq.scan around minimum 10MHz res.
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.03	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	300.	200.	0.03	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	800.	1024.	1.5								
% digrate	2.										


% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 35.53	380.	2.*10^6	200.	1.	1980.	1.	{1.,18.7115,36.1442}





%%%%%%%%%%%%%%%
% B=0mT wide range frEq.scan 50MHz res. (currently appendix?)
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.244	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	500.	200.	0.244	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	1200.	1024.	1.5								
% digrate	2.										

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 26.	4.	1.*10^6	50.	1.	30.	2.	{1.,18.7115,36.1442}


%%%%%%%%%%%%%%%
% B=38mT nnn pair peak
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.03	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	500.	200.	0.03	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	1200.	1024.	1.5								
% digrate	2.										

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 35.53	380.	2.*10^6	200.	1.	41.	1.	{1.,18.7115,36.1442}



%%%%%%%%%%%%%%%
% B=0mT AF and FM nn and nnn pair peaks
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.014	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	500.	200.	0.014	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	1200.	1024.	1.5								
% digrate	2.										

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 36.97	4.	2.*10^6	200.	1.	41.	1.	{1.,18.7115,36.1442}

% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.014	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	500.	200.	0.014	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	1200.	1024.	1.5								
% digrate	2.										

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 36.54	4.	2.*10^6	200.	1.	41.	1.	{1.,18.7115,36.1442}

% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.027	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	500.	200.	0.027	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	1200.	1024.	1.5								
% digrate	2.										

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 35.8	4.	2.*10^6	200.	1.	41.	1.	{1.,18.7115,36.1442}

% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.029	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	500.	200.	0.029	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	1200.	1024.	1.5								
% digrate	2.										

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 35.44	4.	2.*10^6	200.	1.	41.	1.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% B=38mT x=0.1% envelopes as fct. of frEq. (Fig 3 a)
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.184	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	500.	200.	0.184	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	1200.	1024.	1.5								
% digrate	2.										


% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 27.04	380.	1.*10^6	20.	1.	200.	0.	{1.,18.7115,36.1442}


%%%%%%%%%%%%%%%
% B=38mT x=0.01% main peak frEq.sweep (Fig 3 e inset)
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	chirp	0.	100.	0.18	1.5	3.	 - 	 - 	 - 	0.0161	0.
% pi	chirp	1000.	200.	0.18	1.5	3.	 - 	 - 	 - 	0.0161	0.
% det	2200.	8192.	1.5								
% digrate	2.										


% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 27.8	380.	2.*10^6	100.	1.	151.	1.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% B=38mT x=0.01% envelopes as fct. of frEq. (Fig 3 e)
%%%%%%%%%%%%%%%

% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	chirp	0.	25.	0.15	1.5	3.	 - 	 - 	 - 	0.0161	0.
% pi	chirp	400.	50.	0.15	1.5	3.	 - 	 - 	 - 	0.0161	0.
% det	850.	2048.	1.5								
% digrate	2.										

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 27.89	380.	2.*10^6	100.	1.	25500.	0.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% B=38mT x=0.1%iso High SNR traces Main peak and side
%%%%%%%%%%%%%%%
% Main
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.27	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	350.	200.	0.27	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	900.	2048.	1.5								
% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 27.8	379.	2.*10^6	100.	10.	100.	2.	{1.,18.7115,36.1442}

% Main side
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.24	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	350.	200.	0.24	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	900.	2048.	1.5								
% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 27.98	379.	2.*10^6	100.	10.	100.	2.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% B=38mT x=0.1%iso High SNR trace NNN pair peak 100/200ns pulses
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	100.	0.005	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	350.	200.	0.005	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	900.	2048.	1.5								


% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 35.535	379.	2.*10^6	100.	10.	100.	2.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% B=38mT x=0.1%iso High SNR trace NNN pair peak 10/20ns pulses
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	10.	0.05	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	280.	20.	0.05	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	580.	2048.	1.5								
% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 35.535	379.	2.*10^6	100.	10.	100.	0.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% B=0mT x=0.1%iso High SNR trace "main"
%%%%%%%%%%%%%%%

% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	20.	0.77	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	280.	40.	0.77	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	600.	2048.	1.5								

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 28.26	0.	2.*10^6	100.	20.	50.	2.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% B=0mT x=0.1%iso High SNR trace FM NNN peak
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	10.	0.39	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	280.	20.	0.39	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	580.	2048.	1.5								

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 35.425	0.	2.*10^6	100.	20.	50.	1.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% B=0mT x=0.1%iso High SNR trace AF NNN peak
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	Gausscascade	0.	10.	0.39	1.5	3.	1.	0.5	0.4	0.0161	0.
% pi	Gausscascade	280.	20.	0.39	1.5	3.	1.	0.5	0.4	0.0161	0.
% det	580.	2048.	1.5								

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 35.825	0.	2.*10^6	100.	20.	50.	1.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% CPMG B=38mT x=0.1%iso Main peak
%%%%%%%%%%%%%%%
% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	chirp	0.	20.	0.58	1.5	3.	 - 	 - 	 - 	0.0161	0.
% pi	chirp	270.	40.	0.58	1.5	3.	 - 	 - 	 - 	0.0161	0.
% det	550.	1024.	1.5								
% digrate	2.										

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 27.8	379.	2.*10^6	10.	1.	1920.	2.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% CPMG B=38mT x=0.1%iso NNN pair peak
%%%%%%%%%%%%%%%

% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	chirp	0.	2.	0.11	1.5	3.	 - 	 - 	 - 	0.0161	0.
% pi	chirp	279.	4.	0.11	1.5	3.	 - 	 - 	 - 	0.0161	0.
% det	559.	1024.	1.5								
% digrate	2.										

% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 35.535	379.	2.*10^6	20.	1.	1920.	0.	{1.,18.7115,36.1442}

%%%%%%%%%%%%%%%
% Appendix
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
% All four "butterfly" measurements of 0.01%iso around B=0
%%%%%%%%%%%%%%%

% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	chirp	0.	100.	0.13	1.5	3.	Missing[KeyAbsent,A_n1]	Missing[KeyAbsent,x_n1]	Missing[KeyAbsent,deltax_n1]	0.0161	0.
% pi	chirp	400.	200.	0.13	1.5	3.	Missing[KeyAbsent,A_n2]	Missing[KeyAbsent,x_n2]	Missing[KeyAbsent,deltax_n2]	0.0161	0.
% det	1000.	2048.	1.5								
% digrate	2.										


% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 28.05	2.	2.*10^6	200.	1.	1176.	0.	{1.,18.7115,36.1442}


% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	chirp	0.	100.	0.13	1.5	3.	Missing[KeyAbsent,A_n1]	Missing[KeyAbsent,x_n1]	Missing[KeyAbsent,deltax_n1]	0.0161	0.
% pi	chirp	400.	200.	0.13	1.5	3.	Missing[KeyAbsent,A_n2]	Missing[KeyAbsent,x_n2]	Missing[KeyAbsent,deltax_n2]	0.0161	0.
% det	1000.	2048.	1.5								
% digrate	2.										


% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 28.05	9.	2.*10^6	200.	1.	2296.	0.	{1.,18.7115,36.1442}


% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	chirp	0.	100.	0.13	1.5	3.	Missing[KeyAbsent,A_n1]	Missing[KeyAbsent,x_n1]	Missing[KeyAbsent,deltax_n1]	0.0161	0.
% pi	chirp	400.	200.	0.13	1.5	3.	Missing[KeyAbsent,A_n2]	Missing[KeyAbsent,x_n2]	Missing[KeyAbsent,deltax_n2]	0.0161	0.
% det	1000.	2048.	1.5								
% digrate	2.										


% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 28.05	24.	2.*10^6	200.	1.	3416.	0.	{1.,18.7115,36.1442}


% name	type	t	tp	scale	nu_init	channel	A_n	x_n	deltax_n	Qshift	phase
% pi/2	chirp	0.	100.	0.04	1.5	3.	Missing[KeyAbsent,A_n1]	Missing[KeyAbsent,x_n1]	Missing[KeyAbsent,deltax_n1]	0.0161	0.
% pi	chirp	400.	200.	0.04	1.5	3.	Missing[KeyAbsent,A_n2]	Missing[KeyAbsent,x_n2]	Missing[KeyAbsent,deltax_n2]	0.0161	0.
% det	1000.	2048.	1.5								
% digrate	2.										


% freq	B	reptime	shots	avgs	Ntot	IFgain	IFgain_levels
% 29.425	2.	2.*10^6	200.	1.	3416.	0.	{1.,18.7115,36.1442}
